GroundNLQ @ Ego4D Natural Language Queries Challenge 2023

In this report, we present our champion solution for Ego4D Natural Language Queries (NLQ) Challenge in CVPR 2023. Essentially, to accurately ground in a video, an effective egocentric feature extractor and a powerful grounding model are required. Motivated by this, we leverage a two-stage pre-training strategy to train egocentric feature extractors and the grounding model on video narrations, and further fine-tune the model on annotated data. In addition, we introduce a novel grounding model GroundNLQ, which employs a multi-modal multi-scale grounding module for effective video and text fusion and various temporal intervals, especially for long videos. On the blind test set, GroundNLQ achieves 25.67 and 18.18 for R1@IoU=0.3 and R1@IoU=0.5, respectively, and surpasses all other teams by a noticeable margin. Our code will be released at\url{https://github.com/houzhijian/GroundNLQ}.

==> Table/leaderboard.tex <==
% Table generated by Excel2LaTeX from sheet 'mainresult'
\begin{table}[htbp]
  \centering
  \caption*{Performance comparison of the top three teams on the public leaderboard.}
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{c|cccc}
    \toprule
    Team name &  R1 @0.3 & R1 @0.5 & R5 @0.3 & R5 @0.5 \\
    \midrule
    ego-env & 23.28 & 14.36 & 27.25 & 17.58 \\
    asl\_nlq & 24.13 & 15.46 & 34.37 & 23.18 \\
    GroundNLQ & 25.67 & 18.18 & 42.05 & 29.80 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:leaderboard}%
\end{table}%

